Perspectives on How To Conduct Responsible Anti-Human Trafficking Research in Operations and Analytics

Human trafficking, the commercial exploitation of individuals, is a gross violation of human rights and harms societies, economies, health and development. The related disciplines of Operations Management (OM), Analytics, and Operations Research (OR) are uniquely positioned to support trafficking prevention and intervention efforts by efficiently evaluating a plethora of decision alternatives, and providing quantitative, actionable insights. As operations and analytical efforts in the counter-trafficking field emerge, it is imperative to grasp subtle yet distinctive nuances associated with human trafficking. This note is intended to inform those practitioners working in the field by highlighting key features of human trafficking activity. We grouped nine themes around three broad categories: (1) representation of human trafficking, (2) consideration of survivors and communities, and (3) analytics related. These insights are derived from our collective experience in working in this area and substantiated by domain expertise.

==> backup_content.tex <==
%\documentclass[review]{elsarticle}
%
%
%\usepackage{lscape}
%\usepackage{lineno}
%\usepackage{hyperref}
%\usepackage{natbib}
%\usepackage[colorinlistoftodos]{todonotes}
%
%
%\journal{European Journal of Operational Research} 
%
%
%%%%%%%%%%%%%%%%%%%%%%%%
%%% Elsevier bibliography styles
%%%%%%%%%%%%%%%%%%%%%%%%
%
%%% To change the style, put a % in front of the second line of the current style and
%%% remove the % from the second line of the style you would like to use.
%%%%%%%%%%%%%%%%%%%%%%%%
%
%%% Numbered
%%\bibliographystyle{model1-num-names}
%%\bibliography{HTRespRes}
%
%%% Numbered without titles
%%\bibliographystyle{model1a-num-names}
%
%%% Harvard
%%\bibliographystyle{model2-names.bst}\biboptions{authoryear}
%
%%% Vancouver numbered
%%\usepackage{numcompress}\bibliographystyle{model3-num-names}
%
%%% Vancouver name/year
%%\usepackage{numcompress}\bibliographystyle{model4-names}\biboptions{authoryear}
%
%%% APA style
% \bibliographystyle{model5-names}\biboptions{authoryear}
%%\usepackage{natbib}
%\usepackage[natbib = true]{biblatex}
%\bibliography{HTRespRes}
%
%%% AMA style
%%\usepackage{numcompress}\bibliographystyle{model6-num-names}
%
%%% `Elsevier LaTeX' style
%
%%\bibliographystyle{elsarticle-num}
%
%%\usepackage{natbib}
%% \biboptions{numbers,sort&compress}
%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%
%
%\begin{document}
%
%\begin{frontmatter}
